Novel Factorization Strategies for Higher Order Tensors: Implications for Compression and Recovery of Multi-linear Data

In this paper we propose novel methods for compression and recovery of multilinear data under limited sampling. We exploit the recently proposed tensor- Singular Value Decomposition (t-SVD)[1], which is a group theoretic framework for tensor decomposition. In contrast to popular existing tensor decomposition techniques such as higher-order SVD (HOSVD), t-SVD has optimality properties similar to the truncated SVD for matrices. Based on t-SVD, we first construct novel tensor-rank like measures to characterize informational and structural complexity of multilinear data. Following that we outline a complexity penalized algorithm for tensor completion from missing entries. As an application, 3-D and 4-D (color) video data compression and recovery are considered. We show that videos with linear camera motion can be represented more efficiently using t-SVD compared to traditional approaches based on vectorizing or flattening of the tensors. Application of the proposed tensor completion algorithm for video recovery from missing entries is shown to yield a superior performance over existing methods. In conclusion we point out several research directions and implications to online prediction of multilinear data.

==> IterativeAlgorithms.tex <==
\subsection{Algorithms for solving the optimization problems}
For these two problems we discussed above, in the original domain, the incomplete data is a sampling of $\T{M}$ and the sampling tensor is $P_\bold{\Omega}$. In other words, let $\T{Y}$ be the available (sampled) data, then
\begin{equation}
\T{Y} = P_\bold{\Omega} \T{M}
\end{equation} 
\noindent then take the Fourier transform along the third dimension to the both sides we get
\begin{equation}
\hat{\T{Y}} = \mathscr{F}_3 (P_\bold{\Omega} \T{M})
\end{equation}
where $\mathscr{F}$ is the operator representing the Fourier transform along the third dimension of tensors. Let $\mathscr{F}^{-1}$ be the inverse Fourier transform along the third dimension, and rewrite the equation as
\begin{equation}
\hat{\T{Y}} = \mathscr{F}_3 P_\bold{\Omega} \mathscr{F}_{3}^{-1} (\hat{\T{M}})
\end{equation}
\noindent where $\hat{\T{M}}$ is the tensor after taking Fourier transform along the third dimension of $\T{M}$. Define $\mathcal{G}=\mathscr{F}_3 P_\bold{\Omega} \mathscr{F}_{3}^{-1}$, then what we have is
\begin{equation}
\hat{\T{Y}} = \mathcal{G} (\hat{\T{M}}) \\
\end{equation}


We essentially use Alternating Direction Method of Multipliers (ADMM), \cite{Boyd_Eckstein}. To be complete here we present the details of the algorithm. Following \cite{Boys_Eckstein} one can re-write the optimization problem 
\begin{align}
\min ||\hat{\T{X}}||_{TNN} \\
s.t. \hat{\T{Y}} = {\cal G}(\T{X}) 
\end{align}
equivalently as follows 
\begin{align}
\min ||\hat{\T{Z}}||_{TNN} + \mathbf{1}_{\hat{\T{Y}} = {\cal G}(\hat{\T{X}})} \\
s.t.\,\,\, \hat{\T{X}} - \hat{\T{Z}} = 0  
\end{align}
The following the general framework of ADMM and using operator splitting techniques, \cite{Eckstein93} we have the following recursion, 
\begin{align}
\label{eq:proj}
\hat{\T{X}}^{(k+1)}& = \arg\min_{\hat{\T{X}}} \left\{ \mathbf{1}_{\T{Y} = {\cal G}(\hat{\T{X}})} + \langle \T{Q}^{(k)}, \hat{\T{X}} \rangle  + \frac{1}{2} || \hat{\T{X}} - \hat{\T{Z}}^{(k)}||_{2}^{2} \right\}\nonumber \\
& = \arg\min_{\hat{\T{X}}: \T{Y} = {\cal G}(\hat{\T{X}})} \left\{|| \hat{\T{X}} - (\hat{\T{Z}}^{(k)} - \T{Q}^{k})||_{2}^{2} \right\}\\
\label{eq:shrink}
\hat{\T{Z}}^{k+1}    & = \arg \min_{\T{Z}} \left\{ \frac{1}{\rho} ||\hat{\T{Z}}||_{TNN} + \frac{1}{2} ||  \hat{\T{Z}} - (\hat{\T{X}}^{k+1} + \T{Q}^{k})||_{2}^{2} \right\}\\
\T{Q}^{k+1} &= \T{Q}^{k} + \left(\hat{\T{X}}^{k+1} - \hat{\T{Z}}^{k+1}\right)
\end{align}
where Equation~(\ref{eq:proj}) is least-squares projection onto the constraint and the solution to Equation~(\ref{eq:shrink}) is given by the singular value thresholding, \cite{Watson,Candes,Cai}. In the actual implementation only this step is performed in the Fourier domain while all the the other steps can be done in the original domain. If the data is positive one can enforce an additional projection onto the positive cone. We will like to further remark on the shrinkage operation. It can be shown that the shrinkage operation in the Fourier domain on the singular values of each of the faces is equivalent to performing a \emph{tubal shrinkage} via convolution. 

==> Submitted version/Conclusion.tex <==
\section{Future work - collaborative filtering of multi-linear data}
\label{sec:future_work}
\vspace{-2mm} 
Our work has direct implications to study prediction and recovery of \emph{multi-linear} signals. For example, similar to the scenario of \emph{collaborative filtering} with bounded trace norm for 2-D matrices considered in \cite{Hazan_JMLR12}, one can consider a multi-linear version of the problem and look at collaborative filtering with bounded tensor norms which in turn are derived from the particular tensor decomposition, namely the t-SVD. Due to its optimality properties as well as algebraic grounding, one can look for similar identifiability results similar to the matrix case. Extension of our algorithm in Section \ref{sec:tcompletion} to address this sequential online setting for collaborative filtering of multi-linear data and providing provably optimal learning guarantees is an important research direction. 

%In this paper, we invented 2 new tensor rank and its application on tensor completion. We propose the theoretical foundations of tensor-nuclear-norm as well as the algorithms to solve tensor completion problems using this tensor-nuclear-norm minimization method. Then we did some analysis to the sampling rate requirement of our algorithm comparing to the traditional nuclear norm minimization. Then we showed our algorithm is better than LRTC and traditional nuclear norm minimization in several video experiments. 
%
%However, the proposed tensor completion algorithm requires that the data is of low tubal rank in our sense. Sometimes it may not fit the certain application. Also tensor-tubal-norm is a much more proper norm to represent the tensor-tubal-rank but we haven't finish the proof of the norm itself. After proving we can try using the similar ADMM frame work on applications. 

==> Submitted version/Introduction.tex <==
\section{Introduction}
\vspace{-2mm} 
This paper focuses on several novel methods for robust recovery of multilinear signals or tensors (essentially viewed as 2-D, 3-D,..., N-D data) under limited sampling and measurements. Signal recovery from partial measurements, sometimes also referred to as the problem of data completion for specific choice of measurement operator being a simple downsampling operation, has been an important area of research, not only for statistical signal processing problems related to inversion, \cite{Ely_ICASSP2013, Wright12-II,Ji_PAMI12}, but also in machine learning for online prediction of ratings, \cite{Hazan_JMLR12}. All of these applications exploit low structural and informational complexity of the data, expressed either as low rank for the 2-D matrices \cite{Ely_ICASSP2013,Wright12-II}, which can be extended to higher order data via \emph{flattenning or vectorizing} of the tensor data such as tensor N-rank \cite{GandyRY2011}, or other more general tensor-rank measures based on particular tensor decompositions such as higher oder SVD (HOSVD) or Tucker-3 and Canonical Decomposition (CANDECOMP). See \cite{SIREV} for a survey of these decompositions.

The key idea behind these methods is that under the assumption of low-rank of the underlying data thereby constraining the complexity of the hypothesis space, it should be feasible to recover data (or equivalently predict the missing entries) from number of measurements in proportion to the rank. Such analysis and the corresponding identifiability results are obtained by considering an appropriate complexity penalized recovery algorithm under observation constraints, where the measure of complexity, related to the notion of rank, comes from a particular \emph{factorization} of the data. Such algorithms are inherently combinatorial and to alleviate this difficulty one looks for the tightest convex relaxations of the complexity measure, following which the well developed machinery of convex optimization as well as convex analysis can be employed to study the related problem. For example, rank of the 2-D matrix being relaxed to the Schatten 1-norm, \cite{Watson92} and tensor $N$-rank for order $N > 2$ tensors being relaxed to overlapped Schatten p-norms, \cite{GandyRY2011}. Similarly one can extend this approach to HOSVD and take the sum of absolute values of the entries of the core tensor as a (relaxed) measure of data complexity.

Note that all of the current approaches to handle multilinear data extend the nearly optimal 2-D SVD\footnote{Optimality of 2-D SVD is based on the optimality of truncated SVD as the best $k$-dimensional $\ell_2$ approximation.} based vector space approach to the higher order ($N > 2$) case. This results in loss of optimality in the representation.  In contrast, our approach is based upon recent results on decomposition/factorization of tensors in \cite{Braman2010,KilmerMartin2010,KilmerBramanHao2011} in which the authors refer to as tensor-SVD or t-SVD for short. In the t-SVD framework we view 3D tensors as a matrix of tubes (in the third dimension) and define a commutative operation (convolution) between the tubes. This commutative structure leads to viewing the tensor tensor multiplication as a simple matrix-matrix multiplication where the multiplication operation is defined via the commutative operation. With this construction, one can now introduce the notion of a t-SVD which is similar to the traditional SVD, see Figure~\ref{fig:tSVD}. In this context we identify two (relaxed) measures of structural complexity, namely the Tensor-Nuclear-Norm (TNN) first used in \cite{semerci1} for multi-energy CT application and Tensor Tubal Norm (TTN) which extends the notion of SVD based rank to the number of non-zero singular tubes in t-SVD. 

This paper is organized as follows. Section \ref{sec:tSVD} presents the notations and provide an overview and key results on t-SVD from \cite{Braman2010, KilmerMartin2010, KilmerBramanHao2011} and illustrates the key differences and advantages over other tensor decomposition methods. We will propose measures of structural complexity based on t-SVD. Using these measures, in Section \ref{sec:tcompletion} we introduce a complexity penalized algorithm for tensor completion from randomly sampled data cube. As an application we consider video data completion from missing entries and Section \ref{sec:video_app} shows the compression performance of t-SVD based representation on several video data sets and evaluates the performance of the proposed algorithm for video completion then compares it to current approaches. Finally we outline implications of this work and future research directions in Section \ref{sec:future_work}.

%================================================================================%%%
%This construction leads to viewing a multilinear data as a module of oriented matrices $\in \Real^{n_1\times 1 \times n_3}$ over a commutative ring with identity formed of the tubes $\in \Real^{1\times 1 \times n_3$ and in this
%First, the t-SVD unlike the HOSVD and CANDECOMP is not \emph{orientation invariant}, i.e. it depends upon the orientation of the tensor. In this regard this view of a tensor shares similarity with other approaches to study tensors such as tensor n-rank  \cite{} which is the sum of ranks of various \emph{unfoldings} of the tensors along different directions. Nevertheless, as pointed out in \cite{}, one can associate a notion of rank of a tensor in terms of t-SVD which as we will show in this paper can be more meaningful for some data types. \\
%For tensor completion from limited data we exploit the fact that the data has low structural complexity. These measures of structural complexity are based on the t-SVD and are essentially equivalent to nuclear norms used in matrix completion methods \cite{} and tensor n-rank used in tensor completion methods \cite{}. One of these measures namely the tensor nuclear norm (TNN) was proposed and used for multi-energy CT imaging in \cite{Oguz}. In this paper we propose another related measure (we cannot call it a norm yet) and show that for some problems it may be right measure of structural complexity of multilinear data. For the case of TNN we extend the results for matrix completion in \cite{Candes} to tensor completion and outline an iterative shrinkage algorithm for tensor completion. \\
%================================================================================%%%

%================================================================================%%%
%A large number of signal processing problems involve the manipulation of quantities of which the elements are addressed by more than 2 indices. Compared to the vectors (first order) and matrices (second order) , these higher-order stuff are called higher-order tensors. So the term \emph{tensor}, which are used throughout the paper, is a multi-dimensional array of numbers. For example, $A \in \mathrm{R}^{n_1 \times n_2 \times n_3}$ , then we say $A$ is a third-order tensor. In the following , when we say a tensor, we mean a 3-dimensional array of numbers.
%Tensors arise in a wide variety of application areas which includes but is not limited to, chemometrics, psychometrics, image and signal processing. There are various tensor decompositions nowadays such as CANDECOMP/PARAFAC(CP), TUCKER, and High-Order SVD. They all give us a linear algebra tool to this multilinear area. but the main idea remains the same. raising the salad bar. one of the main ideas in the thoery of matrix completion is the 
%The recent work by  have provided some familiar tools of linear algebra can be extended to better understanding in the third-order tensors. We discuss a matrix completion here in the sense of third-order tensor singular value decomposition (TSVD). A similar shrinkage algorithm is extended on the third-order tensors. We investigate a new notation of the rank in third-order tensor case and do theoretical analysis on that, then give out an algorithm for solving matrix completion problem using this algorithm. We conclude with examples in video to see how this algorithm works in application.
%================================================================================%%%

==> Submitted version/IterativeAlgorithms.tex <==
\subsection{Algorithms for solving the optimization problems}
For these two problems we discussed above, in the original domain, the incomplete data is a sampling of $\T{M}$ and the sampling tensor is $P_\bold{\Omega}$. In other words, let $\T{Y}$ be the available (sampled) data, then
\begin{equation}
\T{Y} = P_\bold{\Omega} \T{M}
\end{equation} 
\noindent then take the Fourier transform along the third dimension to the both sides we get
\begin{equation}
\hat{\T{Y}} = \mathscr{F}_3 (P_\bold{\Omega} \T{M})
\end{equation}
where $\mathscr{F}$ is the operator representing the Fourier transform along the third dimension of tensors. Let $\mathscr{F}^{-1}$ be the inverse Fourier transform along the third dimension, and rewrite the equation as
\begin{equation}
\hat{\T{Y}} = \mathscr{F}_3 P_\bold{\Omega} \mathscr{F}_{3}^{-1} (\hat{\T{M}})
\end{equation}
\noindent where $\hat{\T{M}}$ is the tensor after taking Fourier transform along the third dimension of $\T{M}$. Define $\mathcal{G}=\mathscr{F}_3 P_\bold{\Omega} \mathscr{F}_{3}^{-1}$, then what we have is
\begin{equation}
\hat{\T{Y}} = \mathcal{G} (\hat{\T{M}}) \\
\end{equation}


We essentially use Alternating Direction Method of Multipliers (ADMM), \cite{Boyd_Eckstein}. To be complete here we present the details of the algorithm. Following \cite{Boys_Eckstein} one can re-write the optimization problem 
\begin{align}
\min ||\hat{\T{X}}||_{TNN} \\
s.t. \hat{\T{Y}} = {\cal G}(\T{X}) 
\end{align}
equivalently as follows 
\begin{align}
\min ||\hat{\T{Z}}||_{TNN} + \mathbf{1}_{\hat{\T{Y}} = {\cal G}(\hat{\T{X}})} \\
s.t.\,\,\, \hat{\T{X}} - \hat{\T{Z}} = 0  
\end{align}
The following the general framework of ADMM and using operator splitting techniques, \cite{Eckstein93} we have the following recursion, 
\begin{align}
\label{eq:proj}
\hat{\T{X}}^{(k+1)}& = \arg\min_{\hat{\T{X}}} \left\{ \mathbf{1}_{\T{Y} = {\cal G}(\hat{\T{X}})} + \langle \T{Q}^{(k)}, \hat{\T{X}} \rangle  + \frac{1}{2} || \hat{\T{X}} - \hat{\T{Z}}^{(k)}||_{2}^{2} \right\}\nonumber \\
& = \arg\min_{\hat{\T{X}}: \T{Y} = {\cal G}(\hat{\T{X}})} \left\{|| \hat{\T{X}} - (\hat{\T{Z}}^{(k)} - \T{Q}^{k})||_{2}^{2} \right\}\\
\label{eq:shrink}
\hat{\T{Z}}^{k+1}    & = \arg \min_{\T{Z}} \left\{ \frac{1}{\rho} ||\hat{\T{Z}}||_{TNN} + \frac{1}{2} ||  \hat{\T{Z}} - (\hat{\T{X}}^{k+1} + \T{Q}^{k})||_{2}^{2} \right\}\\
\T{Q}^{k+1} &= \T{Q}^{k} + \left(\hat{\T{X}}^{k+1} - \hat{\T{Z}}^{k+1}\right)
\end{align}
where Equation~(\ref{eq:proj}) is least-squares projection onto the constraint and the solution to Equation~(\ref{eq:shrink}) is given by the singular value thresholding, \cite{Watson,Candes,Cai}. In the actual implementation only this step is performed in the Fourier domain while all the the other steps can be done in the original domain. If the data is positive one can enforce an additional projection onto the positive cone. We will like to further remark on the shrinkage operation. It can be shown that the shrinkage operation in the Fourier domain on the singular values of each of the faces is equivalent to performing a \emph{tubal shrinkage} via convolution. 

==> Submitted version/PerformanceEvaluation.tex <==
\vspace{-2mm} 
\subsection{Performance evaluation of video data completion}
%We now show the performance evaluation on several candidate data sets of the proposed tensor completion algorithms exploiting the complexity in the tSVD decomposition. 
\vspace{-2mm} 
%\subsection{Results A}
\input{PerformanceEvaluation_Jamie}
%\subsection{Results B}
%\input{PerformanceEvaluation_Greg}

==> Submitted version/PerformanceEvaluation_Jamie.tex <==
In this part we test 3 algorithms for video data completion from randomly missing entries:  TNN minimization of Section \ref{sec:tcompletion}, Low Rank Tensor Completion (LRTC) algorithm in \cite{Ji_PAMI12}, which uses the notion of tensor-n-rank \cite{GandyRY2011}, and the nuclear norm minimization on the vectorized video data using the algorithm in \cite{Cai_SVT}. As an application of the t-SVD to higher order tensor we also show performance on a 4-D color Basketball video data of size $144 \times 256 \times 3 \times 80$. 
%It is a 4th order tensor and we can use tSVD to decompose this tensor then get the recovery similarly using LRTC and tensor-nuclear-norm minimization. 

Figures ~\ref{fig:recovery} and \ref{fig:basketball_color} show the results of recovery using the 3 algorithms. Figure~\ref{fig:recovery_rse} shows the RSE (dB) plots for sampling rates ranging from $10\%$ to $90\%$ where the sampling rate is defined to be the percentage of pixels which are known. Results from the figures show that the TNN minimization algorithm gives excellent reconstruction over the LRTC and Nuclear norm minimization.  These results are in line with the compressibility results in Section~\ref{sec:compression}.

\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c c }
      \includegraphics[width = .22\textwidth]{figs/recovery_figs/basketball_color_10_sample.png}  \hspace{2mm}
      \includegraphics[width = .22\textwidth]{figs/recovery_figs/basketball_color_10_LRTC.png}     \hspace{2mm}
      \includegraphics[width = .22\textwidth]{figs/recovery_figs/basketball_color_10_TNN.png} \\
      \end{tabular}}
  \caption{ Recovery for color basketball video: \textbf{Left}: Sampled Video($10\%$). \textbf{Middle}: LRTC recovery. \textbf{Right}: Tensor-nuclear-norm minimization recovery }
\label{fig:basketball_color}
\end{figure}    

\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c }
    \includegraphics[width = .45\textwidth]{figs/merl_error.png} \hspace{5mm}
    \includegraphics[width = .45\textwidth]{figs/basketball_error.png}
    \end{tabular}}
  \caption{ RSE (dB) plot against sampling rate \textbf{Left}: MERL video. \textbf{Right}: Basketball video }
\label{fig:recovery_rse}
\end{figure}    



==> Submitted version/ProblemSetUp_0523_Jamie.tex <==
\section{Tensor completion/prediction from missing observations}
\vspace{-2mm} 
\label{sec:tcompletion}
We will show the case when the tensor data is simply decimated randomly or down sampled in this section. Specifically we consider the problem of data completion from missing entries for multilinear signals.  Suppose there is an unknown tensor $\T{M}$ of size $n_1 \times n_2 \times n_3$ which is {\bf \emph{assumed to have a low tubal-rank}} and we are given a subset of entries $ \{ \T{M}_{ijk}:(i,j,k) \in \bold{\Omega} \}$ where $\bold{\Omega}$ is an indicator tensor of size $n_1 \times n_2 \times n_3$. Our objective is to recover the entire $\T{M}$. This section develops an algorithm for addressing this problem via solving the following complexity penalized algorithm:
\begin{equation}
\begin{aligned}
\label{eq:originalTNN}
\mbox{min} \hspace{4mm}&\|\T{X}\|_{TNN} \\
\mbox{subject to } \,\,\,&P_{\bold{\Omega}} ( \T{X} ) = P_{\bold{\Omega}} ( \T{M} )
\end{aligned}
\end{equation}
\noindent where $P_\bold{\Omega}$ is the orthogonal projector onto the span of tensors vanishing outside of $\bold{\Omega}$. So the $(i,j,k)_{th}$ component of $ P_{\bold{\Omega}} ( \T{X} )$ is equal to $\T{M}_{ijk}$ if $(i,j,k) \in \bold{\Omega}$ and zero otherwise. Let $\T{Y}$ be the available (sampled) data: $\T{Y} = P_\bold{\Omega} \T{M}$. Define $\mathcal{G}=\mathscr{F}_3 P_\bold{\Omega} \mathscr{F}_{3}^{-1}$ where $\mathscr{F}_3$ and $\mathscr{F}^{-1}_3$ are the operators representing the Fourier and inverse Fourier transform along the third dimension of tensors. Then we have
$\hat{\T{Y}} = \mathcal{G} (\hat{\T{M}})$ where $\hat{\T{Y}}$ and $\hat{\T{M}}$ are the Fourier transforms of $\T{Y}$ and $\T{M}$ along the third mode.
%In the original domain, the incomplete data is a sampling of $\T{M}$ and the sampling tensor is $P_\bold{\Omega}$. In other words, let $\T{Y}$ be the available (sampled) data, then $\T{Y} = P_\bold{\Omega} \T{M}$. Take the Fourier transform along the third dimension to the both sides we get $\hat{\T{Y}} = \mathscr{F}_3 (P_\bold{\Omega} \T{M})$, where $\mathscr{F}$ is the operator representing the Fourier transform along the third dimension of tensors. Let $\mathscr{F}^{-1}_3$ be the inverse Fourier transform along the third dimension and $\hat{\T{M}}$ be the tensor after taking Fourier transform along the third dimension of $\T{M}$. So the equation becomes $\hat{\T{Y}} = \mathscr{F}_3 P_\bold{\Omega} \mathscr{F}_{3}^{-1} (\hat{\T{M}})$. 
So (\ref{eq:originalTNN}) is equivalent with the following:
\begin{equation}
\begin{aligned}
\label{eq:fourierdomain_min}
\mbox{min} \hspace{4mm}&||\mbox{blkdiag}(\hat{\T{X}}) ||_*\\
\mbox{subject to } \,\,\,\,\,&\hat{\T{Y}} = {\cal G}(\hat{\T{X}}) 
\end{aligned}
\end{equation}
where $\hat{\T{X}}$ is the Fourier transform of $\T{X}$ along the third dimension and $\text{blkdiag}(\hat{\T{X}})$ is defined in (\ref{eq:blkdiag}). Noting that $\|\T{X}\|_{TNN} = ||\text{blkdiag}(\hat{\T{X}}) ||_*$. To solve the optimization problem, one can re-write (\ref{eq:fourierdomain_min}) equivalently as follows: 
\begin{equation}
\begin{aligned}
\min \hspace{4mm}& ||\text{blkdiag}( \hat{\T{Z}} )||_* + \mathbf{1}_{\hat{\T{Y}} = {\cal G}(\hat{\T{X}})} \\
\mbox{subject to } \,\,\,\,\, &\hat{\T{X}} - \hat{\T{Z}} = 0  
\end{aligned}
\end{equation}
where $\mathbf{1}$ denotes the indicator function. Then using the general framework of Alternating Direction Method of Multipliers(ADMM)\cite{Boyd_ADMM} we have the following recursion, 
\begin{align}
\label{eq:proj}
\hat{\T{X}}^{k+1}& = \arg\min_{\hat{\T{X}}} \left\{ \mathbf{1}_{\T{Y} = {\cal G}(\hat{\T{X}})} + \langle \hat{\T{Q}}^{k}, \hat{\T{X}} \rangle  + \frac{1}{2} || \hat{\T{X}} - \hat{\T{Z}}^{k}||_{2}^{2} \right\}\nonumber \\
& = \arg\min_{\hat{\T{X}}: \T{Y} = {\cal G}(\hat{\T{X}})} \left\{|| \hat{\T{X}} - (\hat{\T{Z}}^{k} - \hat{\T{Q}}^{k})||_{2}^{2} \right\}\\
\label{eq:shrink}
\hat{\T{Z}}^{k+1}    & = \arg \min_{\T{Z}} \left\{ \frac{1}{\rho} ||\text{blkdiag}(\hat{\T{Z}})||_* + \frac{1}{2} ||  \hat{\T{Z}} - (\hat{\T{X}}^{k+1} + \hat{\T{Q}}^{k})||_{2}^{2} \right\}\\
\hat{\T{Q}}^{k+1} &= \hat{\T{Q}}^{k} + \left(\hat{\T{X}}^{k+1} - \hat{\T{Z}}^{k+1}\right)
\end{align}
where Equation~(\ref{eq:proj}) is least-squares projection onto the constraint and the solution to Equation~(\ref{eq:shrink}) is given by the singular value thresholding\cite{Watson92,Cai_SVT}. 

\textbf{Equivalence of the algorithm to \emph{iterative singular-tubal shrinkage via convolution}}:
According to the particular format that (\ref{eq:shrink}) has, we can break it up into $n_3$ independent minimization problems. Let $\hat{\T{Z}}^{k+1,(i)}$ denotes the $i_{th}$ frontal slice of $\hat{\T{Z}}^{k+1}$. Similarly define $\hat{\T{X}}^{k+1,(i)}$ and $\hat{\T{Q}}^{k,(i)}$. Then (\ref{eq:shrink}) can be separated as:
\begin{equation}
\begin{aligned}
\label{eq:shrink2}
\hat{\T{Z}}^{k+1,(i)}   & = \arg \min_{W} \left\{ \frac{1}{\rho} ||W||_* + \frac{1}{2} ||  W - (\hat{\T{X}}^{k+1,(i)} + \hat{\T{Q}}^{k,(i)})||_{2}^{2} \right\}
\end{aligned}
\end{equation}
for $i = 1,2,...,n_3$. This means each $i_{th}$ frontal slice of $\hat{\T{Z}}^{k+1}$ can be calculated through (\ref{eq:shrink2}). The solution to (\ref{eq:shrink2}) can be found in\cite{Watson92,Cai_SVT}. In detail, if $U S V^\text{T} = (\hat{\T{X}}^{k+1,(i)} + \hat{\T{Q}}^{k,(i)})$ is the SVD of $(\hat{\T{X}}^{k+1,(i)} + \hat{\T{Q}}^{k,(i)})$, then the solution to (\ref{eq:shrink2}) is $U D_\tau (S) V^\text{T}$, where $D_\tau (S) = \text{diag}(S_{i,i} - \tau)_+$ for some positive constant $\tau$ and $``+"$ means keeping the positive part. This is equivalent to multiplying $(1-\frac{\tau}{S_{i,i}})_+$ to the $i_{th}$ singular value of $S$. So each frontal slice of $\hat{\T{Z}}^{k+1}$ can be calculated using this shrinkage on each frontal slice of $(\hat{\T{X}}^{k+1} + \hat{\T{Q}}^{k})$. Let  $\T{U} * \T{S}* \T{V}^\text{T} = (\T{X}^{k+1} + \T{Q}^{k})$ be the t-SVD of $(\T{X}^{k+1} + \T{Q}^{k})$ and $\hat{\T{S}}$ be the Fourier transform of $\T{S}$ along the third dimension. Then each element of the singular tubes of $\hat{\T{Z}}^{k+1}$ is the result of multiplying every entry $\hat{\T{S}}(i,i,j)$ with $(1-\frac{\tau}{\hat{\T{S}}(i,i,j)})_+$ for some $\tau > 0$. Since this process is carried out in the Fourier domain, in the original domain it is equivalent to convolving each tube $\T{S}(i,i,:)$ of $\T{S}$ with a real valued tubal vector $\vec{\tau}_i$ which is the inverse Fourier transform of the vector $[ ( 1-\frac{\tau_{i}(1)}{\hat{\T{S}}(i,i,1)})_+ , ( 1-\frac{\tau_{i}(2)}{\hat{\T{S}}(i,i,2)})_+ , ... , ( 1-\frac{\tau_{i}(n_3)}{\hat{\T{S}}(i,i,n_3)})_+ ]$. This operation can be captured by $\T{S}*\T{T}$, where $\T{T}$ is an f-diagonal tensor with $i_{th}$ diagonal tube to be $\vec{\tau}_i$. Then  $\T{Z}^{k+1} = \T{U}* ( \T{S}*\T{T} )* \T{V}^\text{T}$. In summary, the shrinkage operation in the Fourier domain on the singular values of each of the frontal faces is equivalent to performing a \emph{tubal shrinkage} via convolution in the original domain.


%In the actual implementation only this step is performed in the Fourier domain while all the the other steps can be done in the original domain. If the data is positive one can enforce an additional projection onto the positive cone. We will like to further remark on the shrinkage operation. It can be shown that the shrinkage operation in the Fourier domain on the singular values of each of the faces is equivalent to performing a \emph{tubal shrinkage} via convolution. 




==> Submitted version/compress.tex <==
\vspace{-2mm} 
\subsection{Compressibility of multi-linear data using t-SVD}
\vspace{-2mm} 
\label{sec:compression}
%In this section we are going to show two tSVD based data compression methods, and give some comparison results between our methods and the well-studied SVD based matrix compression technique. It turns out that some kinds of data are more compact in the proposed multilinear representation than traditional approach. Particularly we will examine some video data with stationary and non-stationary camera motion.
We outline two methods for compression based on t-SVD and compare them with the traditional truncated SVD based approach in this section. Note that we don't compare with truncated HOSVD or other tensor decompositions as there is no notion of optimality for these decompositions in contrast to truncated t-SVD and truncated SVD. 

The use of SVD in matrix compression has been widely studied in \cite{1093309} and \cite{465543}. 
%Given a low rank matrix, or this matrix can be approximated very well by a low rank matrix, then SVD can be used to find this approximation. 
For a matrix $A \in \Real^{m \times n}$ with its SVD $A = USV^T$, the rank $r$ approximation of $A$ is the matrix $A_r = U_r S_r V^\text{T}_r$, where $S_r$ is a $r \times r$ diagonal matrix with $S_r(i,i) = S(i,i), i = 1,2,...,r$. $U_r$ consists of the first $r$ columns of $U$ and $V^\text{T}_r$ consists of the first $r$ rows of $V^\text{T}_r$. The compression is measured by the ratio of the total number of entries in $A$, which is $mn$, to the total number of entries in $U_r$, $S_r$ and $V^\text{T}_r$, which is equal to $(m+n+1)r$. Extending this approach to a third-order tensor $\T{M}$ of size $n_1 \times n_2 \times n_3$, we vectorize each frontal slice and save it as a column, so we get an $n_1 n_2 \times n_3$ matrix. Then the compression ratio of rank $k_1$ SVD approximation is 
\begin{align}
\text{ratio}_{\text{SVD}} = \frac{n_1 n_2 n_3}{n_1 n_2 k_1 + k_1 + n_3 k_1} = \frac{n_1 n_2 n_3}{k_1(n_1 n_2 +n_3+1)}
\end{align}
where $1 \le k_1 \le \text{min}(n_1n_2,n_3)$. Generally even with small $k_1$, the approximation $M_{k_1}$ gets most of the information of $\T{M}$. 

{\bf Method 1} : Based on t-SVD our first method for compression, which we call t-SVD compression, basically follows the same idea of truncated SVD but in the \emph{Fourier domain}. For an $n_1 \times n_2 \times n_3$ tensor $\T{M}$, we use Algorithm 1 to get $\hat{\T{M}}$, $\hat{\T{U}}$, $\hat{\T{S}}$ and $\hat{\T{V}}^\text{T}$. It is known that $\hat{\T{S}}$ is a f-diagonal tensor with each frontal slice is a diagonal matrix. So the total number of f-diagonal entries of $\hat{\T{S}}$ is $n_0 n_3$ where $n_0 = \text{min} (n_1,n_2)$.  We choose an integer $k_2$, $1 \le k_2 \le n_0 n_3$ and keep the $k_2$ largest f-diagonal entries of $\hat{\T{S}}$ then set the rest to be $0$. If $\hat{\T{S}}(i,i,j)$ is set to be $0$, then let the corresponding columns $\hat{\T{U}}(:,i,j)$ and $\hat{\T{V}}^\text{T}(:,i,j)$ also be $0$. We then call the resulting tensors $\hat{\T{U}}_{k_2}$, $\hat{\T{S}}_{k_2}$ and $\hat{\T{V}}^\text{T}_{k_2}$. So the approximation is $\T{M}_{k_2} = \T{U}_{k_2} * \T{S}_{k_2} * \T{V}^\text{T}_{k_2}$ where $\T{U}_{k_2}$, $\T{S}_{k_2}$ and $\T{V^\text{T}}_{k_2}$ are the inverse Fourier transforms of $\hat{\T{U}}_{k_2}$, $\hat{\T{S}}_{k_2}$ and $\hat{\T{V}}^\text{T}_{k_2}$  along the third dimension.  
%Noting that the in order to get a real reconstruction from the Fourier domain using the inverse Fourier transform, the choice of $k_1$ has to depend on $n_3$ because of the symmetric property of Fourier transform. Since is $\T{S}(i,i,j) = \bar{\T{S}}(i,i,n_3+2-j), then if $\T{S}(i,i,j)$ is picked however $\T{S}(i,i,j)$ is not, then the reconstruction is going to be complex. In order to guarantee this we only need to ensure that singular values which has same value should be both kept or both set to 0.%
The compression ratio rate for this method is
\begin{align}
\text{ratio}_\text{t-SVD} = \frac{n_1 n_2 n_3}{(n_1 \times \frac{k_2}{n_3} + n_2 \times \frac{k_2}{n_3} +\frac{k_2}{n_3}) \times n_3} = \frac{n_1 n_2 n_3}{k_2(n_1+n_2+1)}
\end{align}
where $1 \le k_2 \le n_0 n_3$.

{\bf Method 2}:  Our second method for compressing is called t-SVD-tubal compression and is also similar to truncated SVD but in the \emph{t-product} domain. As in \textbf{Theorem 2.3.1}, we take the first $k_3$ tubes $ ( 1\le k_3 \le n_0) $ in $\T{S}$ and get the approximation $\T{M}_{k_3} = \sum_{i=1}^{k_3} \T{U}(:,i,:) * \T{S}(i,i,:) * \T{V}(:,i,:)^\text{T} $.

%For a $n_1 \times n_2 \times n_3$ tensor $\T{M}$, the tSVD is: $\T{M} = \T{U}*\T{S}*\T{V}^\text{T}$. Different from SVD which takes $r$ singular values, we will take first $k_3$ tubes $ ( 1\le k_3 \le n_0) $ in $\T{S}$ and set the rest $n_0 - k_3$ tubes to be zero. Correspondingly set the last $n_0 - k_3$ lateral slices of $\T{U}$ and  the last $n_0 - k_3$ horizontal slices of $\T{V}^\text{T}$ to be zero. Call the tensors after doing this to be $\T{U}_{k_3}$, $\T{S}_{k_3}$ and $\T{V}^\text{T}_{k_3}$. The approximation for this method is $\T{M}_{k_3} = \T{U}_{k_3} * \T{S}_{k_3} * \T{V}^\text{T}_{k_3}$.
Compression ratio rate for the second method is 
\begin{align}
\text{ratio}_\text{t-SVD-tubal} = \frac{n_1 n_2 n_3}{(n_1 k_3 + n_2 k_3 + k_3)n_3} = \frac{n_1 n_2}{k_3(n_1 + n_2 +1)}
\end{align}
where $1 \le k_3 \le n_0$.



%\begin{figure}[htbp]
%\centering \makebox[0in]{
%    \begin{tabular}{c c c}
%      \includegraphics[width = .17\textwidth]{figs/escalator_frame15.png}
%      
%      \includegraphics[width = .17\textwidth]{figs/merl_frame30.png}
%      
%      \includegraphics[width = .17\textwidth]{figs/basketball_frame20.png}
%      
%      \end{tabular}}
%  \caption{Three testing videos: escalator video, MERL video and basketball video. }
%\label{fig:original}
%\end{figure}


\begin{figure}[h]
\centering \makebox[0in]{
    \begin{tabular}{c c}
    \includegraphics[width = .16\textwidth]{figs/escalator_frame15.png}
      \includegraphics[width = .16\textwidth]{figs/merl_frame30.png}
      \includegraphics[width = .16\textwidth]{figs/basketball_frame20.png}&
      \includegraphics[width = .16\textwidth]{figs/compress_figs/escalator_SVD.png}  
      \includegraphics[width = .16\textwidth]{figs/compress_figs/escalator_12.png} 
      \includegraphics[width = .16\textwidth]{figs/compress_figs/escalator_11.png} \\
      (a) & (b) \\
      \includegraphics[width = .16\textwidth]{figs/compress_figs/merl_SVD.png}
      \includegraphics[width = .16\textwidth]{figs/compress_figs/merl_12.png}
      \includegraphics[width = .16\textwidth]{figs/compress_figs/merl_11.png} &
      \includegraphics[width = .16\textwidth]{figs/compress_figs/basketball_SVD.png}
      \includegraphics[width = .16\textwidth]{figs/compress_figs/basketball_12.png}
      \includegraphics[width = .16\textwidth]{figs/compress_figs/basketball_11.png} \\
      (c) & (d) 
      \end{tabular}}
  \caption{ (\textbf{a}) Three testing videos: escalator video, MERL video and basketball video. (b) (c) (d) are compression results under compression ratio 5. For (b) (c) (d) from left to right: SVD compression, t-SVD-tubal compression and t-SVD compression}
\label{fig:compress_recovery}
\end{figure}
We now illustrate the performance of SVD based compression, t-SVD compression and t-SVD tubal compression on 3 video datasets shown in Figure~\ref{fig:compress_recovery}-(a).
\vspace{-2mm}
\begin{enumerate}
\itemsep0em
\item The first video, referred to as the Escalator video, (source: http://www.ugcs.caltech.edu/~srbecker/rpca.shtml\#2 ) of size $130 \times 160 \times 50$ (length $\times$ width $\times$ frames) from a stationary camera. %Stationary camera means the background of each frame stays the same throughout the video. The motion in the video are people walking and escalator running which only take small part of the screen. This kind of property gives us very high correlation between any two frames of the data. 
\item The second video, referred to as the MERL video, is a {\bf \emph{time lapse video}} of size $192 \times 256 \times 38$ also from a stationary camera ({\bf data courtesy}: Dr. Amit Agrawal, Mitsubishi Electric Research Labs (MERL), Cambridge, MA). 
\item The third video, referred to as the Basketball video is a $144 \times 256 \times 80$ video (source: YouTube) with a  {\bf \emph{non-stationary panning camera}} moving from left to right horizontally following the running players. 
\end{enumerate}
\vspace{-2mm}
Figure~\ref{fig:compress_recovery} (b) to (d) show the compression results for the 3 videos when truncated according to vectorized SVD and t-SVD compression (method 1) and t-SVD tensor tubal compression (method 2). In Figure~\ref{fig:compress_rse} we show the relative square error (RSE) comparison for different compression ratio where RSE is defined in dB as $\text{RSE} = 20 \log_{10} ( \|\T{X}_{\text{rec}} - \T{X}\|_\text{F} / \|\T{X}\|_\text{F} )$. In all of the 3 results, the performance of t-SVD compression (method 1) is the best. This implies that tensor multi-rank fits very well for video datasets from both stationary and non-stationary cameras. SVD compression method (based on vectorization) has a better performance over the t-SVD-tubal compression on the Escalator and MERL video. %The reason for this is that these two videos are taken by stationary cameras, so the two matrix representations of the videos have lower rank in traditional sense than the tensor tubal-rank. Even the motions of shadows and clouds in merl video data are huge, stationary camera plays a more important role here. 
However, t-SVD tubal compression (method 2) works much better than SVD compression on the Basketball video. This is because in the videos where the camera is panning or in motion, one frontal slice of the tensor to the next frontal slice can be effectively represented as a shift and scaling operation which in turn is captured by a convolution type operation and t-SVD is based on such an operation along the third dimension.

%The reason that t-SVD compression always work better than t-SVD tubal-compression is because t-SVD compression is more flexible on the choice of singular values. For example, for one diagonal tube of $\T{S}$, t-SVD compression method could keep some large entries and throw the small ones. However, t-SVD-tubal compression method can only keep the whole tube or throw it.


%We will now show some examples where using the truncated tSVD dubbed as T-SVD for data compression yields superior results compared to the truncated SVD (which is the only other known computationally feasible method which is  shown to be optimal). 
%
%We will now outline several cases where we will show by means of direct calculation that certain kinds of data are more compact in the proposed multilinear representation than traditional approaches.   In particular we will examine video with stationary \& non-stationary camera motion and MRI volumetric data. 
%
% In general data appears to be well compressible in the tSVD domain if the sequence from one frontal slice to the next frontal slice can be represented as a shift and scaling operation.  A subset of the class of representation is convolution by a time shifted delta function which describes the change in a position of a static image from frame to frame.  
%
%Do demonstrate the compressibility of the tSVD we generated a contrived example of a static image moved within a larger field of view (figure \ref{fig:contrived_example}).  In this example a $26 \times 26$ image was moved downward a single pixel within a larger image of 100 by 100 pixels.  The movement was then repeated 100 times to generate a 100 by 100 by 100 volumetric data cube.   The truncated tSVD was then applied to the data and total number of terms used to represent the cube was recorded.  This process was then repeated for the standard SVD where each frontal slice or frame was reshaped into a vector of length 100,000 to generate a matrix of size 100,000 by 100.  From figure \ref{fig:contrived_example} we can clearly see that the data is poorly compressed in the SVD domain as the shift operation from column to column will result in a high increase in rank of the matrix.  However, the tSVD is able to compress the sequence with a high degree of accuracy in a fraction of terms.    Therefore, we believe that data that has shifted but repeating structures from slice to slice can be will compressed in the tSVD domain.  In order to demonstrate this we will look at two examples of non-stationary camera motion.  In which the moving foreground and background can be well represented by the tSVD. 
%\subsubsection{Escalator Reconstruction}
%Repeat with escalator data, 

\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c c}
      \includegraphics[width = .33\textwidth]{figs/compress_figs/escalator.png}
      
      \includegraphics[width = .33\textwidth]{figs/compress_figs/merl.png}
      
      \includegraphics[width = .33\textwidth]{figs/compress_figs/basketball.png}
      
      \end{tabular}}
  \caption{ Compression ratio and RSE comparison for 3 videos.}
\label{fig:compress_rse}
\end{figure}


%
%\begin{figure}[htbp]
%\centering \makebox[0in]{
%    \begin{tabular}{c c}
%      \includegraphics[width = .5\textwidth]{figs/compress_escalator_2.png}
%      
%      \includegraphics[width = .5\textwidth]{figs/compress_escalator.png}
%      \end{tabular}}
% \caption{Escalator Video Results}
%  \label{fig:compress_escalator}
%\end{figure}

\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c c c }
      \includegraphics[width = .20\textwidth]{figs/recovery_figs/merl_20_sample.png}  
      \includegraphics[width = .20\textwidth]{figs/recovery_figs/merl_20_nuclear.png}      
      \includegraphics[width = .20\textwidth]{figs/recovery_figs/merl_20_LRTC.png}      
      \includegraphics[width = .20\textwidth]{figs/recovery_figs/merl_20_TNN.png} \\     
   
      \includegraphics[width = .20\textwidth]{figs/recovery_figs/basketball_20_sample.png}     
      \includegraphics[width = .20\textwidth]{figs/recovery_figs/basketball_20_nuclear.png}    
      \includegraphics[width = .20\textwidth]{figs/recovery_figs/basketball_20_LRTC.png}     
      \includegraphics[width = .20\textwidth]{figs/recovery_figs/basketball_20_TNN.png} 
      \end{tabular}}
  \caption{ Compression results for MERL and Basketball video. From left to right: Sampled video($20\%$), Nuclear norm minimization (vectorization and SVD based) result, LRTC result, TNN minimization result. \textbf{First row}: MERL video. \textbf{Second row}: Basketball video.}
\label{fig:recovery}
\end{figure}


==> Submitted version/macrofile.tex <==
%% ----------------------------------------------------------------------
%% Definitions, Macros, Etc.
%% ----------------------------------------------------------------------

%% Hyper-linked References
\newcommand{\Sec}[1]{\hyperref[sec:#1]{\S\ref*{sec:#1}}} %section
\newcommand{\Eqn}[1]{\hyperref[eq:#1]{(\ref*{eq:#1})}} %equation
\newcommand{\Fig}[1]{\hyperref[fig:#1]{Figure~\ref*{fig:#1}}} %figure
\newcommand{\Tab}[1]{\hyperref[tab:#1]{Table~\ref*{tab:#1}}} %table
\newcommand{\Thm}[1]{\hyperref[thm:#1]{Theorem~\ref*{thm:#1}}} %theorem
\newcommand{\Lem}[1]{\hyperref[lem:#1]{Lemma~\ref*{lem:#1}}} %lemma
\newcommand{\Prop}[1]{\hyperref[prop:#1]{Property~\ref*{prop:#1}}} %property
\newcommand{\Cor}[1]{\hyperref[cor:#1]{Corollary~\ref*{cor:#1}}} %corollary
\newcommand{\Def}[1]{\hyperref[def:#1]{Definition~\ref*{def:#1}}} %definition
\newcommand{\Alg}[1]{\hyperref[alg:#1]{Algorithm~\ref*{alg:#1}}} %algorithm
\newcommand{\Ex}[1]{\hyperref[ex:#1]{Example~\ref*{ex:#1}}} %example

% Theorem-like constructs
%\newtheorem{example}[theorem]{Example}

% Blackboard fonts
\newcommand{\Real}{\mathbb{R}}

%% Transposes
\newcommand{\Tra}{^{\rm T}} % Transpose
\newcommand{\Cct}{^\dagger} % Complex conjugate transpose

%% Permutation index
\newcommand{\bfpp}{{\bf p}_n}

%% Matrix & Tensor Operations
\newcommand{\Circ}[1]{{\rm circ}\left( #1 \right)}
\newcommand{\Fold}[1]{{\rm fold}\left( #1 \right)}
\newcommand{\Unfold}[1]{{\rm unfold}\left( #1 \right)}
\newcommand{\Twist}[1]{{\rm twist}(\M{#1})}
\newcommand{\Squeeze}[1]{{\rm squeeze}(#1)}
\newcommand{\squeeze}{{\rm squeeze}}
\newcommand{\Mout}{\diamondsuit}
\newcommand{\circu}{ {\rm circ}}
\newcommand{\bcirc}{ {\rm bcirc}}
\newcommand{\vvec}{ {\rm vec}}

%% Element of complicated object that is surrounded by parens
\newcommand{\PE}[2]{\left( #1 \right)_{#2}}

%% Vector notation
\newcommand{\V}[1]{{\bm{\mathbf{\MakeLowercase{#1}}}}} % vector
\newcommand{\VE}[2]{\MakeLowercase{#1}_{#2}} % vector element

%% Matrix notation
\newcommand{\M}[1]{{\bm{\mathbf{\MakeUppercase{#1}}}}} % matrix
\newcommand{\Mhat}[1]{{\bm{\hat \mathbf{\MakeUppercase{#1}}}}} % matrix
\newcommand{\Mbar}[1]{{\bm{\bar \mathbf{\MakeUppercase{#1}}}}} % matrix
\newcommand{\ME}[2]{\MakeLowercase{#1}_{#2}} % matrix element
\newcommand{\MC}[2]{\V{#1}_{#2}}

%% Tensor notation
\newcommand{\T}[1]{\boldsymbol{\mathscr{\MakeUppercase{#1}}}} %tensor
\newcommand{\TLS}[2]{\M{#1}_{[#2]}} % lateral slice
\newcommand{\TFS}[2]{\M{#1}_{#2}} % frontal slice
\newcommand{\TT}[2]{\V{#1}_{#2}} % tube
\newcommand{\TE}[2]{\MakeLowercase{#1}_{#2}} % tensor element


%% Shortcuts
\newcommand{\TA}{\T{A}}
\newcommand{\TB}{\T{B}}
\newcommand{\TS}{\T{S}}
\newcommand{\TC}{\T{C}}
\newcommand{\TU}{\T{U}}
\newcommand{\TV}{\T{V}}
\newcommand{\TG}{\T{G}}

\newcommand{\Vu}{\V{u}}
\newcommand{\Vv}{\V{v}}
\newcommand{\Vq}{\V{q}}
\newcommand{\Vr}{\V{r}}
\newcommand{\Vp}{\V{p}}
\newcommand{\Vd}{\V{d}}
\newcommand{\Vzz}{\V{z}}
\newcommand{\Vb}{\V{b}}
\newcommand{\Vg}{\V{g}}
\newcommand{\Vh}{\V{h}}
\newcommand{\MH}{\M{H}}
\newcommand{\MG}{\M{G}}
\newcommand{\MA}{\M{A}}
\newcommand{\MX}{\M{X}}
\newcommand{\MZ}{\M{Z}}
\newcommand{\MW}{\M{W}}
%\newcommand{\TD}{\T{D}}

\newcommand{\SaS}{{\mathcal S}}

\newcommand{\MGC}{\tilde{\MG}}

\newcommand{\Matlab}{{\sc Matlab}\xspace}
\newcommand{\matlab}{{\sc Matlab}\xspace}
\newcommand{\qtext}[1]{\quad\text{#1}\quad}

\newcommand{\matvec}{{\tt Vec}}
\newcommand{\fld}{{\tt Fold}}

\def \bK{\mathbf{K}}
\def \bF{\mathbf{F}}
\def \bD{\mathbf{D}}
\def \bB{\mathbf{B}}
\def \bA{\mathbf{A}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}

%\newcommand{\bea}{\left[ \begin{array}}
%\newcommand{\eea}{ \end{array} \right]} 

\newcommand{\bftheta}{ {\boldsymbol \theta}}
\newcommand{\bfrho}{ {\boldsymbol \rho}}
\newcommand{\bfeta}{ {\boldsymbol \eta}}
\newcommand{\fft}{ \mbox{\tt fft} }
\newcommand{\ifft}{ \mbox{\tt ifft} }



==> Submitted version/tSVD_Ning_Aeron_05_14_2013_NH_gte.tex <==

\section{Brief overview of t-SVD}
\label{sec:tSVD}
\vspace{-2mm} 
In this section, we describe the tensor decomposition as proposed in \cite{Braman2010,KilmerMartin2010,KilmerBramanHao2011} and the notations used throughout the paper. 
\vspace{-2mm} 
\subsection{Notation and Indexing}
\vspace{-2mm} 
A \emph{\textbf{Slice}} of an N-dimensional tensor is a 2-D section defined by fixing all but two indices. A \emph{\textbf{Fiber}} of an N-dimensional tensor is a 1-D section defined by fixing all indices but one \cite{SIREV}. For a third order tensor $\T{A}$, we will use the Matlab notation $\T{A}(k,:,:)$ , $\T{A}(:,k,:)$ and $\T{A}(:,:,k)$ to denote the $k_{th}$ horizontal, lateral and frontal slices, and $\T{A}(:,i,j)$, $\T{A}(i,:,j)$ and $\T{A}(i,j,:)$ to denote the $(i,j)_{th}$ mode-1, mode-2 and mode-3 fiber.  In particular, we use $\T{A}^{(k)}$ to represent $\T{A}(:,:,k)$.
\begin{defn}
\emph{\textbf{Tensor Transpose}}.  Let $\T{A}$ be a tensor of size $n_1 \times n_2 \times n_3$, then $\T{A} \Tra$ is the $n_2 \times n_1 \times n_3$ tensor obtained by transposing each of the frontal slices and then reversing the order of transposed frontal slices $2$ through $n_3$.
\end{defn}
\begin{defn} \emph{\textbf{Identity Tensor}}. The identity tensor $\T{I} \in \mathbb{R}^{n_1 \times n_1 \times n_3}$ is a tensor whose first frontal slice is the $n_1 \times n_1$ identity matrix and  all other frontal slices are zero.
\end{defn}
\begin{defn} \emph{\textbf{f-diagonal Tensor}}. A tensor is called f-diagonal if each frontal slice of the tensor is a diagonal matrix.
\end{defn}
We can view a 3-D tensor of size $n_1 \times n_2 \times n_3$ as an $n_1 \times n_2$ matrix of tubes. By introducing a commutative operation $*$ between the tubes $\mathbf{a}, \mathbf{b}\in \Real^{1 \times 1 \times n_3}$  via $\mathbf{a} * \mathbf{b} = \mathbf{a} \circ \mathbf{b}$ where $\circ$ denotes the \emph{circular convolution} between the two vectors, we can define the t-product between two tensors.  This multiplication is analogous to the matrix multiplication except that circular convolution replaces the multiplication operation between the elements (which are tubes now).
\begin{defn} \emph{\textbf{t-product}}.  
The t-product $\T{C}$ of $\T{A} \in \mathbb{R}^{n_1 \times n_2 \times n_3}$ and $\T{B} \in \mathbb{R}^{n_2\times n_4 \times n_3}$ is a tensor of size $n_1 \times n_4 \times n_3$ where the $(i,j)_{th}$ tube denoted by $\T{C}(i,j,:)$ for $i = 1,2, ..., n_1$ and $j = 1, 2,..., n_4$ of the tensor $\T{C}$ is given by $\sum_{k=1}^{n_2} \T{A}(i,k,:) * \T{B}(k,j,:)$.
\end{defn}
%With the fact that the block circulant matrices can be block diagonalized by applying Fourier transform \cite{gvl:mat, HaoKilmerBramanHoover2012}, i.e.
%\begin{equation}
%\begin{aligned}
%(F_{n_3} \otimes I_{n_1})  \bcirc{ ( \T{A} ) } (F_{n_3}^{\rm{H}} \otimes I_{n_2}) 
%=  \rm{blockdiag} (\hat{ \T{A}}^{(1)} , \cdots , \hat{\T{A}}^{(n_3)} ) 
%= 
%\begin{bmatrix}
%\hat{\T{A}}^{(1)} & 0 & \cdots & 0 \\
%0 & \hat{\T{A}}^{(2)} & \cdots & 0 \\
%\vdots & \ddots & \ddots & \vdots \\
%0 & \cdots & 0 & \hat{\T{A}}^{(n_3)}
%\end{bmatrix} 
%\end{aligned}
%\end{equation}
The t-product of $\T{A}$ and $\T{B}$ can be computed efficiently by performing the fast Fourier transformation (FFT) along the tube fibers of $\T{A}$ and $\T{B}$ to get $\hat{\T{A}}$ and $\hat{\T{B}}$,  multiplying the each pair of the frontal slices of $\hat{\T{A}}$ and $\hat{\T{B}}$ to obtain $\hat{\T{C}}$, and then taking the inverse FFT along the third mode to get the result. For details about the computation, see \cite{KilmerMartin2010, KilmerBramanHooverHao, HaoKilmerBramanHoover2012}.
\begin{defn} \emph{\textbf{Orthogonal Tensor}}. A tensor $\T{Q}\in\mathbb{R}^{n_1\times n_1\times n_3}$ is orthogonal if
\begin{equation}
\T{Q} \Tra * \T{Q} = \T{Q} * \T{Q} \Tra  = \T{I}
\end{equation}
\end{defn}

\subsection{Tensor Singular Value Decomposition (t-SVD)}
\vspace{-2mm} 
The new t-product  allows us to define a tensor Singular Value Decomposition (t-SVD). % Based on the  t-product as defined above we can define tensor singular value decomposition (tSVD) as follows.
\begin{theorem}
For $\T{M}\in\mathbb{R}^{n_1 \times n_2 \times n_3}$, the t-SVD of $\T{M}$ is  given by
\begin{equation}
\T{M} = \T{U} *\T {S} *\T{V}\Tra
\end{equation}
\noindent where $\T{U}$ and $\TV$ are orthogonal tensors of size $n_1 \times n_1 \times n_3 $ and  $n_2 \times n_2 \times n_3 $ respectively. $\T{S}$ is a rectangular $f$-diagonal tensor of size $n_1 \times n_2 \times n_3 $, and $*$ denotes the t-product. 
\end{theorem}
\vspace{-1.5mm}
We can obtain this decomposition by computing matrix SVDs in the Fourier domain, see Algorithm 1. The notation in the algorithm can be found in\cite{Martin_SIAM2013}. %({bf: NB} - where $\T{D}(:,:,i)$ is the $i$-th slice of the tensor $\T{D}$ in terms of Matlab storage \& notiation\cite{KilmerMartin2010}), taken from \cite{KilmerMartin2010} for a general $N$-D tensor,
Figure \ref{fig:tSVD} illustrates the decomposition for the 3-D case.
\begin{algorithm}
\label{alg:tSVD - for $N$-D tensor}
  \caption{t-SVD}
  \begin{algorithmic}
  \STATE \textbf{Input: } $\T{M} \in \mathbb{R}^{n_1 \times n_2  ... \times n_N}$
  %\STATE \textbf{Output: } $\T{C}:= \T{A}*\T{B} \in \mathbb{R}^{n_1 \times \l  \times n_3 ... \times n_M}$.
  \STATE $\rho = n_3n_4...n_N$
   \FOR{$i = 3 \hspace{2mm} \rm{to} \hspace{2mm} N$}
  	\STATE ${\T{D}} \leftarrow \rm{fft}(\T{M},[\hspace{1mm}],i)$;
  \ENDFOR
  
  \FOR{$i = 1 \hspace{2mm} \rm{to} \hspace{2mm} \rho$}
  	\STATE $ [\M{U}, \M{S}, \M{V}] = svd(\T{D}(:,:,i))$
  	\STATE $ {\hat{\T{U}}}(:,:,i) = \M{U}; \hspace{1mm} {\hat{\T{S}}}(:,:,i) = \M{S}; \hspace{1mm} {\hat{\T{V}}}(:,:,i) = \M{V}; $
  \ENDFOR
  
  \FOR{$i = 3 \hspace{2mm} \rm{to} \hspace{2mm} \rho$}
  	\STATE $\T{U} \leftarrow \rm{ifft}(\hat{\T{U}},[\hspace{1mm}],i); \hspace{1mm} \T{S} \leftarrow \rm{ifft}(\hat{\T{S}},[\hspace{1mm}],i); \hspace{1mm} \T{V} \leftarrow \rm{ifft}(\hat{\T{V}},[\hspace{1mm}],)i$;
  \ENDFOR
  \end{algorithmic}
\end{algorithm}


%\begin{algorithm}
%\label{alg:tSVD}
%  \caption{t-SVD}
%  \begin{algorithmic}
%  \STATE \textbf{Input: } $\T{M} \in \mathbb{R}^{n_1 \times n_2  \times n_3}$
%  %\STATE \textbf{Output: } $\T{C}:= \T{A}*\T{B} \in \mathbb{R}^{n_1 \times \l  \times n_3 ... \times n_M}$.
%  %\STATE $\rho = n_3n_4...n_p$
%  % \FOR{$i = 3 \hspace{2mm} \rm{to} \hspace{2mm} p$}
%  	\STATE ${\hat{\T{M}}} \leftarrow \rm{fft}(\T{M},[\hspace{1mm}],3)$;
% % \ENDFOR
%  
%  \FOR{$i = 1 \hspace{2mm} \rm{to} \hspace{2mm} n_3$}
%  	\STATE $ [\M{U}, \M{S}, \M{V}] = svd(\hat{\T{M}}(:,:,i))$
%  	\STATE $ {\hat{\T{U}}}(:,:,i) = \M{U}; \hspace{1mm} {\hat{\T{S}}}(:,:,i) = \M{S}; \hspace{1mm} {\hat{\T{V}}}(:,:,i) = \M{V}; $
%  \ENDFOR
%  
%%  \FOR{$i = 3 \hspace{2mm} \rm{to} \hspace{2mm} p$}
%  	\STATE $\T{U} \leftarrow \rm{ifft}(\hat{\T{U}},[\hspace{1mm}],3); \hspace{1mm} \T{S} \leftarrow \rm{ifft}(\hat{\T{S}},[\hspace{1mm}],3); \hspace{1mm} \T{V} \leftarrow \rm{ifft}(\hat{\T{V}},[\hspace{1mm}],3)$;
%  %\ENDFOR
%  \end{algorithmic}
%\end{algorithm}


\begin{figure}[htbp]
\centering \makebox[0in]{
    \begin{tabular}{c c}
      \includegraphics[scale=0.55]{figs/tSVD.png}
 \end{tabular}}
  \caption{ The t-SVD of an $n_1 \times n_2 \times n_3$ tensor.}
  \label{fig:tSVD}
\end{figure}

\vspace{-2mm} 
\subsection{t-SVD: Fundamental theorems and key results}
\vspace{-2mm} 
The two widely used tensor decompositions, Tucker and PARAFAC\cite{SIREV} are usually seen as a higher order SVD for tensors. Both of these decompositions have several disadvantages. In particular, one cannot  easily determine the rank-one components of the PARAFAC decomposition and given a fixed rank, calculation of an approximation can be  numerically unstable. The tensor-train form of the Tucker decomposition is studied in \cite{Oseledets} as an alternative form. Tucker decomposition can be seen as a generalization of PARAFAC decomposition, and the truncated decomposition doesn't yield the best fit of the original tensor. In contrast, the t-SVD can be easily computed by solving several SVDs in the Fourier domain. More importantly, it gives an optimal approximation of a tensor measured by the Frobenius norm of the difference, as state in the following theorem\cite{KilmerMartin2010, KilmerBramanHooverHao, HaoKilmerBramanHoover2012}. 

\begin{theorem} Let the t-SVD of $\T{M} \in \mathbb{R}^{n_1 \times n_2 \times n_3}$ be 
given by $\T{M} = \T{U} * \T{S} * \T{V}^T$ and for $k < \min(n_1,n_2)$ define
$\T{M}_k = \sum_{i=1}^{k} \T{U}(:,i,:) * \T{S}(i,i,:) * \T{V}(:,i,:)^T $, 
Then
$$\T{M}_k = \arg \min_{\tilde{\T{M}} \in \mathbb{M}} \| \T{M} - \tilde{\T{M}} \|_F $$
where $\mathbb{M} = \{ \T{C} = \T{X} * \T{Y} |
\T{X} \in \mathbb{R}^{n_1 \times k \times n_3}, \T{Y} \in \mathbb{R}^{k 
\times n_2 \times n_3} \}$.
\end{theorem}
\vspace{-2mm} 
\subsection{Measures of tensor complexity using t-SVD }
\vspace{-2mm} 
We  now define two measures of tensor complexity based on the proposed t-SVD: the tensor multi-rank, proposed in  \cite{KilmerBramanHooverHao}, and the novel tensor tubal rank.% using the definitions of the null and range spaces of a tensor as a linear operator on the space (free module) of matrices.  
\begin{defn} \textbf{Tensor multi-rank}. The multi-rank of $\T{A}\in\mathbb{R}^{n_1\times n_2\times n_3}$ is a vector $p$ $\in \Real^{n_3 \times 1}$ with the $i_{th}$ element equal to the rank of the $i_{th}$ frontal slice of $\hat{\T{A}}$ obtained by taking the Fourier transform along the third dimension of the tensor. 
\end{defn}
One can obtain a scalar measure of complexity as the $\ell_1$ norm of the tensor multi-rank. We now define another measure motivated by the matrix SVD. 
%Inspired by the matrix case, another measure can be defined as follows.
\begin{defn} \textbf{Tensor tubal-rank}. The tensor tubal rank of a 3-D tensor is defined to be the number of non-zero tubes of $\T{S}$ in the t-SVD factorization.
\end{defn}
As in the matrix case,  practical applications of these complexity measures require adequate convex relaxations. To this end we have the following result for the Tensor multi-rank. 

\begin{theorem}
The tensor-nuclear-norm (TNN) denoted by $||\T{A}||_{TNN}$ and defined as the sum of the singular values of all the frontal slices of $\hat{\T{A}}$ is a norm and is the tightest convex relaxation to $\ell_1$ norm of the tensor multi-rank.
\end{theorem}
\begin{proof}
\vspace{-3mm}
%\text{rank}(||(F\otimes I)\text{bcirc}(\T{A})(F^\ast\otimes I)||)
The proof that TNN is a valid norm can be found in \cite{semerci1}. The $\ell_1$ norm of the tensor multi-rank is equal to $\text{rank}(\text{blkdiag}(\hat{\T{A}}))$,
%\left(\left[\begin{array}{cccc}\hat{{\bold A}}^{(1)}& & & \\
% & \hat{{\bold A}}^{(2)} & & \\
% & &\ddots & \\
%  & & & \hat{{\bold A}}^{(n)}\end{array} \right]\right)$, 
for which the tightest convex relaxation is the the nuclear norm of  $\text{blkdiag}(\hat{\T{A}})$ which is TNN of $\T{A}$ by definition. Here $\text{blkdiag}(\hat{\T{A}})$ is a block diagonal matrix defined as follows:
% a block diagonal matrix  with $i_{th}$ block equals $\hat{\T{A}}^{(i)}$,$i=1,2,...,n_3$: $\text{blkdiag}(\hat{\T{A}}) = \text{blockdiag}\{  \hat{\T{A}}^{(1)} , \hat{\T{A}}^{(2)} ,..., \hat{\T{A}}^{(n_3)}  \}$.
\begin{equation}
\label{eq:blkdiag}
\text{blkdiag}( \hat{\T{A}} ) = 
  \left[\begin{array}{cccc}\hat{{\T{A}}}^{(1)}& & & \\
 & \hat{{\T{A}}}^{(2)} & & \\
 & &\ddots & \\
  & & & \hat{{\T{A}}}^{(n_3)}\end{array} \right]
\end{equation}
where $\hat{\T{A}}^{(i)}$ is the $i_{th}$ frontal slice of $\hat{\T{A}}$, $i = 1,2,...,n_3$.
\end{proof}
 Similar to the TNN we can seek a relaxation for the tensor-tubal-rank, we call tensor-tubal-norm (TTN). It is defined as the sum of $\ell_2$ norms of the tubes $\T{S}(i,i,:)$. However at this point we haven't proven that the TNN is a norm. Based on simulations and tests on a variety of cases we have the following conjecture.  
\begin{conjecture}
The tensor-tubal-norm is a norm and is the tightest convex relaxation to tensor-tubal-rank.
\end{conjecture}
\vspace{-1.5mm}
We conclude this section with the following important remark. 
\begin{remark}
It may appear that our approach can be generalized by taking any orthogonal transformations along third dimension followed by sampling each slice in the transformed domain. However this perspective cannot be easily extended in the t-SVD  framework, as the notions of transpose does not extend to all transforms. In fact, there is an underlying algebraic framework, namely that of viewing in the third order tensors as linear operators on a \emph{module} \cite{MacLaneBook} of oriented matrices with multiplication defined over a commutative ring with identity \cite{Braman2010}. For sake of brevity we will not discuss these aspects in this paper. 
\end{remark}

